A study on quantum gases: bosons in optical lattices and the one-dimensional interacting Bose gas

Bosonic atoms confined in optical lattices are described by the Bose-Hubbard model and can exist in two different phases, Mott insulator or superfluid, depending on the strength of the system parameters. In the vicinity of the phase boundary, there are degeneracies that occur between every two adjacent Mott lobes. Because of this, nondegenerate perturbation theory fails to give meaningful results for the condensate density: it predicts a phase transition in a point of the phase diagram where no transition occurs. Motivated by this, we develop two different degenerate perturbative methods to solve the degeneracy-related problems. Moreover, we study the one-dimensional repulsively interacting Bose gas under harmonic confinement, with special attention to the asymptotic behavior of the momentum distribution, which is a universal $k^{-4}$ decay characterized by the Tan's contact. The latter constitutes a direct signature of the short-range correlations in such an interacting system and provides valuable insights about the role of the interparticle interactions. We investigate the system constituted of $N$ interacting particles in the strongly interacting limit. In such a regime, the strong interparticle interaction makes the bosons behave similarly to the ideal Fermi gas. Because of the difficulty in analytically solving the system for $N$ particles at finite interaction, the Tonks-Girardeau regime provides a favorable scenario to probe the contact. Therefore, we are able to provide an analytical formula for the Tan's contact. Furthermore, we analyze the scaling properties of the Tan's contact in terms of $N$ in the high-temperature regime as well as in the strongly interacting regime. Finally, we compare our analytical calculations of the Tan's contact to quantum Monte Carlo simulations and discuss some fundamental differences between the canonical and the grand-canonical ensembles.

==> USPSC-IndicesRemissivos.tex <==
%% USPSC-IndicexRemissivos.tex
% ---
% Inicia os Índices Remissivos
% ---
%---------------------------------------------------------------------
% INDICE REMISSIVO
%--------------------------------------------------------------------
\phantompart
\printindex
%---------------------------------------------------------------------


==> USPSC-fichacatalografica.tex <==
% ---
% Inserir a ficha bibliografica
% ---
% Isto é um exemplo de Ficha Catalográfica, ou ``Dados internacionais de
% catalogação-na-publicação''. Você pode utilizar este modelo como referência. 
% Porém, provavelmente a biblioteca da sua universidade lhe fornecerá um PDF
% com a ficha catalográfica definitiva após a defesa do trabalho. Quando estiver
% com o documento, salve-o como PDF no diretório do seu projeto e substitua todo
% o conteúdo de implementação deste arquivo pelo comando abaixo:
%
\begin{fichacatalografica}
	\hspace{-1.4cm}
	\imprimirnotaautorizacao \\ \\
	%\sffamily
	\vspace*{\fill}					% Posição vertical
	\begin{center}					% Minipage Centralizado
		\imprimirnotabib \\
\begin{table}[htb]
	\scriptsize
	\centering	
	\begin{tabular}{|p{0.9cm} p{8.7cm}|}
		\hline
	      & \\
		  &	  \imprimirautorficha     \\
		
		 \imprimircutter & 
							\hspace{0.4cm}\imprimirtitulo~  / ~\imprimirautor~ ;  ~\imprimirorientadorcorpoficha. -- 	\imprimirlocal, \imprimirdata.   \\
		
		  &  % Para incluir nota referente à versão corrigida no corpo da ficha,
			  % incluir % no início da linha acima e tirar a % do início da linha abaixo
			  %	\hspace{0.4cm} \imprimirtitulo~  / ~\imprimirautor~ ; ~\imprimirorientadorcorpoficha~- ~\imprimirnotafolharosto. -- \imprimirlocal, \imprimirdata.  \\
		
			\hspace{0.4cm}\pageref{LastPage} p. : il. (algumas color.) ; 30 cm.\\ 
		  & \\
		  & 
		    \hspace{0.4cm}\imprimirnotaficha ~--~ 
						  \imprimirunidademin, 
						  \imprimiruniversidademin, 
		                  \imprimirdata. \\ 
		  & \\                 
		   % Para incluir nota referente à versão corrigida em notas,
		    % incluir uma % no início da linha acima e	
		    % tirar a % do início da linha abaixo
		    % & \hspace{0.4cm}\imprimirnotafolharosto \\ 
		  & \\ 
		  & \hspace{0.4cm}1. LaTeX. 2. abnTeX. 3. Classe USPSC. 4. Editoração de texto. 5. Normalização da documentação. 6. Tese. 7. Dissertação. 8. Documentos (elaboração). 9. Documentos eletrônicos. I. \imprimirorientadorficha. 
		   II. Título. \\
	
		     %Se houver co-orientador, inclua % antes da linha (antes de II. Título.) 
		     %          e tire a % antes do comando abaixo 
		     %III. Título. \\   
		  \hline
	\end{tabular}
\end{table}
	\end{center}
\end{fichacatalografica}
% ---



==> USPSC-pre-textual-IFSC.tex <==
%% USPSC-pre-textual-IFSC.tex
%% Camandos para definição do tipo de documento (tese ou dissertação), área de concentração, opção, preâmbulo, titulação 
%% referentes ao Programa de Pós-Graduação o IFSC
\instituicao{Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo}
\unidade{INSTITUTO DE F\'ISICA DE S\~AO CARLOS}
\unidademin{Instituto de F\'isica de S\~ao Carlos}
\universidademin{Universidade de S\~ao Paulo}
%\notafolharosto{Vers\~ao original}
%Para versão original em inglês, comente do comando/declaração 
%     acima(inclua % antes do comando acima) e tire a % do 
%     comando/declaração abaixo no idioma do texto
%\notafolharosto{Original version} 
%Para versão corrigida, comente do comando/declaração da 
%     versão original acima (inclua % antes do comando acima) 
%     e tire a % do comando/declaração de um dos comandos 
%     abaixo em conformidade com o idioma do texto
%\notafolharosto{Vers\~ao corrigida \\(Vers\~ao original dispon\'ivel na Unidade que aloja o Programa)}
\notafolharosto{Corrected version \\(Original version available on the Program Unit)}

% ---
% dados complementares para CAPA e FOLHA DE ROSTO
% ---
\universidade{UNIVERSIDADE DE S\~AO PAULO}
\titulo{A study on quantum gases: bosons in optical lattices and the one-dimensional interacting Bose gas}
\titleabstract{Um estudo sobre gases qu\^anticos: b\'osons em redes \'opticas e o g\'as interagente e unidimensional de Bose}
\autor{Felipe Taha Sant'Ana}
\autorficha{Sant'Ana, Felipe Taha}
\autorabr{SANT'ANA, F. T.}

\cutter{S856m}
% Para gerar a ficha catalográfica sem o Código Cutter, basta 
% incluir uma % na linha acima e tirar a % da linha abaixo
%\cutter{ }

\local{S\~ao Carlos}
\data{2020}
% Quando for Orientador, basta incluir uma % antes do comando abaixo
\renewcommand{\orientadorname}{Orientador:}
% Quando for Coorientadora, basta tirar a % utilizar o comando abaixo
%\newcommand{\coorientadorname}{Coorientador:}
\orientador{Prof. Dr. Francisco Ednilson Alves dos Santos}
\orientadorcorpoficha{orientador Francisco Ednilson Alves dos Santos}
\orientadorficha{dos Santos, Francisco Ednilson Alves, orient}
%Se houver co-orientador, inclua % antes das duas linhas (antes dos comandos \orientadorcorpoficha e \orientadorficha) 
%          e tire a % antes dos 3 comandos abaixo
%\coorientador{Prof. Dr. Jo\~ao Alves Serqueira}
%\orientadorcorpoficha{orientadora Elisa Gon\c{c}alves Rodrigues ;  co-orientador Jo\~ao Alves Serqueira}
%\orientadorficha{Rodrigues, Elisa Gon\c{c}alves, orient. II. Serqueira, Jo\~ao Alves, co-orient}

\notaautorizacao{AUTORIZO A REPRODU\c{C}\~AO E DIVULGA\c{C}\~AO TOTAL OU PARCIAL DESTE TRABALHO, POR QUALQUER MEIO CONVENCIONAL OU ELETR\^ONICO PARA FINS DE ESTUDO E PESQUISA, DESDE QUE CITADA A FONTE.}
\notabib{Ficha catalogr\'afica revisada pelo Servi\c{c}o de Biblioteca e Informa\c{c}\~ao Prof. Bernhard Gross, com os dados fornecidos pelo(a) autor(a)}

\newcommand{\programa}[1]{

% DFA ==========================================================================
    \ifthenelse{\equal{#1}{DFA}}{
    	\renewcommand{\areaname}{Concentration area:}
    	\renewcommand{\opcaoname}{Option:}
     	\tipotrabalho{Thesis (Doctor in Science)}
        \area{Theoretical and Experimental Physics}
		%\opcao{Nome da Opção}
        % O preambulo deve conter o tipo do trabalho, o objetivo, 
		% o nome da instituição, a área de concentração e opção quando houver
		\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
		\notaficha{Thesis (Doctorate - Graduate Program in Physics)}
    }{
% MFA ===========================================================================
        \ifthenelse{\equal{#1}{MFA}}{
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica Aplicada}
			%\opcao{Nome da Opção}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
% DFAFC ==========================================================================
    \ifthenelse{\equal{#1}{DFAFC}}{
     	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
        \area{F\'isica Aplicada}
        \opcao{F\'isica Computacional}
        % O preambulo deve conter o tipo do trabalho, o objetivo, 
		% o nome da instituição, a área de concentração e opção quando houver
		\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
		\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% MFAFC ===========================================================================
        \ifthenelse{\equal{#1}{MFAFC}}{
			\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Computacional}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
% DFAFBp ===========================================================================
        \ifthenelse{\equal{#1}{DFAFBp}}{
			\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Biomolecular}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver
			\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
			\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{				
% DFAFBe ===========================================================================
        \ifthenelse{\equal{#1}{DFAFBe}}{
			\renewcommand{\areaname}{Concentration area:}
			\renewcommand{\opcaoname}{Option:}
			\tipotrabalho{Monograph (Doctor in Science)}
	        \area{Basic Physics}
	        \opcao{Biomolecular Physics}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver
			\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
			\notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
        }{				
% MFAFB ===========================================================================
        \ifthenelse{\equal{#1}{MFAFB}}{
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica Aplicada}
	        \opcao{F\'isica Biomolecular}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
        }{
				
% DFB ==========================================================================
    \ifthenelse{\equal{#1}{DFB}}{
     	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
        \area{F\'isica Te\'orica e Experimental}
		%\opcao{Nome da Opção}
        % O preambulo deve conter o tipo do trabalho, o objetivo, 
		% o nome da instituição, a área de concentração e opção quando houver				
		\preambulo{Monografia apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para o Exame de Qualifica\c{c}\~ao, como parte dos requisitos para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
		\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
    }{
% MFB ===========================================================================
        \ifthenelse{\equal{#1}{MFB}}{
	        \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	        \area{F\'isica B\'asica}
			%\opcao{Nome da Opção}
	        % O preambulo deve conter o tipo do trabalho, o objetivo, 
			% o nome da instituição, a área de concentração e opção quando houver				
			\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
			\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
        }{                
% Outros
				\tipotrabalho{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado)}
				\area{Nome da \'Area}
				\opcao{Nome da Op\c{c}\~ao}
		        % O preambulo deve conter o tipo do trabalho, o objetivo, 
				% o nome da instituição, a área de concentração e opção quando houver
				\preambulo{Disserta\c{c}\~ao/Tese apresentada ao Programa de P\'{\o}s-Gradua\c{c}\~ao em F\'{\i}sica do Instituto de F\'{\i}sica de S\~ao Carlos da Universidade de S\~ao Paulo, para obtenç\c{c}\~ao do t\'{\i}tulo de Mestre/Doutor em Ci\^encias.}
				\notaficha{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado - Programa de P\'os-Gradua\c{c}\~ao em Nome da \'Area)}
        }}}}}}}}}}
				
				








==> USPSC-unidades.tex <==
%% USPSC-unidadesTCC.tex
% Camando para definição do programa de Pós-Graduação, Especialidade do Título e Instituição - 21/09/2015
\newcommand{\siglaunidade}[1]{


% EESC-TCC ==========================================================================
    \ifthenelse{\equal{#1}{EESC-TCC}}{
     			\include{USPSC-TCC-pre-textual-EESC}
% ---
    }{
% EESC ==========================================================================
	\ifthenelse{\equal{#1}{EESC}}{
	\include{USPSC-pre-textual-EESC}
	% ---
}{    
% IAU ===========================================================================
        \ifthenelse{\equal{#1}{IAU}}{
        \include{USPSC-pre-textual-IAU}    
        }{
% ICMC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC}}{
        \include{USPSC-pre-textual-ICMC}    
        }{
% IFSC ===========================================================================
        \ifthenelse{\equal{#1}{IFSC}}{
        \include{USPSC-pre-textual-IFSC}    
        }{
% IQSC ===========================================================================
        \ifthenelse{\equal{#1}{IQSC}}{
        \include{USPSC-pre-textual-IQSC}    
        }{

                   
% Outros ========================================================================
                       % ------------------------------------------------------------------------
        \include{USPSC-pre-textual-OUTRO} 
								  }
                }
							}
						}
				}
			}}
         	

